Measurement of the forward-backward asymmetry in low-mass bottom-quark pairs produced in proton-antiproton collisions

We report a measurement of the forward-backward asymmetry, $A_{FB}$, in $b\bar{b}$ pairs produced in proton-antiproton collisions and identified by muons from semileptonic $b$-hadron decays. The event sample was collected at a center-of-mass energy of $\sqrt{s}=1.96$ TeV with the CDF II detector and corresponds to 6.9 fb$^{-1}$ of integrated luminosity. We obtain an integrated asymmetry of $A_{FB}(b\bar{b})=(1.2 \pm 0.7)$\% at the particle level for $b$-quark pairs with invariant mass, $m_{b\bar{b}}$, down to $40$ GeV/$c^2$ and measure the dependence of $A_{FB}(b\bar{b})$ on $m_{b\bar{b}}$. The results are compatible with expectations from the standard model.

==> author.tex <==
% Last update: $Date: 2016/01/04 20:42:12 $
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\affiliation{University of Athens, 157 71 Athens, Greece}
\affiliation{Institut de Fisica d'Altes Energies, ICREA, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\affiliation{Baylor University, Waco, Texas 76798, USA}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\affiliation{University of California, Los Angeles, Los Angeles, California 90024, USA}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\affiliation{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\affiliation{University of Florida, Gainesville, Florida 32611, USA}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\affiliation{Harvard University, Cambridge, Massachusetts 02138, USA}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki, FIN-00014, Helsinki, Finland; Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218, USA}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Karlsruhe Institute of Technology, D-76131 Karlsruhe, Germany}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts 02139, USA}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{Institution for Theoretical and Experimental Physics, ITEP, Moscow 117259, Russia}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131, USA}
\affiliation{The Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Okayama University, Okayama 700-8530, Japan}
\affiliation{Osaka City University, Osaka 558-8585, Japan}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, \ensuremath{^{ll}}University of Padova, I-35131 Padova, Italy}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, USA}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\affiliation{The Rockefeller University, New York, New York 10065, USA}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, \ensuremath{^{rr}}Sapienza Universit\`{a} di Roma, I-00185 Roma, Italy}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\affiliation{Tufts University, Medford, Massachusetts 02155, USA}
\affiliation{Waseda University, Tokyo 169, Japan}
\affiliation{Wayne State University, Detroit, Michigan 48201, USA}
\affiliation{University of Wisconsin-Madison, Madison, Wisconsin 53706, USA}
\affiliation{Yale University, New Haven, Connecticut 06520, USA}

\author{T.~Aaltonen}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki, FIN-00014, Helsinki, Finland; Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{S.~Amerio\ensuremath{^{ll}}}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, \ensuremath{^{ll}}University of Padova, I-35131 Padova, Italy}
\author{D.~Amidei}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{A.~Anastassov\ensuremath{^{w}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Annovi}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{J.~Antos}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{G.~Apollinari}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.A.~Appel}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{T.~Arisawa}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{A.~Artikov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{J.~Asaadi}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{W.~Ashmanskas}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{B.~Auerbach}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\author{A.~Aurisano}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{F.~Azfar}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{W.~Badgett}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{T.~Bae}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{A.~Barbaro-Galtieri}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{V.E.~Barnes}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{B.A.~Barnett}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218, USA}
\author{P.~Barria\ensuremath{^{nn}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{P.~Bartos}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{M.~Bauce\ensuremath{^{ll}}}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, \ensuremath{^{ll}}University of Padova, I-35131 Padova, Italy}
\author{F.~Bedeschi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{S.~Behari}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{G.~Bellettini\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{J.~Bellinger}
\affiliation{University of Wisconsin-Madison, Madison, Wisconsin 53706, USA}
\author{D.~Benjamin}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{A.~Beretvas}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Bhatti}
\affiliation{The Rockefeller University, New York, New York 10065, USA}
\author{K.R.~Bland}
\affiliation{Baylor University, Waco, Texas 76798, USA}
\author{B.~Blumenfeld}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218, USA}
\author{A.~Bocci}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{A.~Bodek}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{D.~Bortoletto}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{J.~Boudreau}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, USA}
\author{A.~Boveia}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{L.~Brigliadori\ensuremath{^{kk}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{C.~Bromberg}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{E.~Brucken}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki, FIN-00014, Helsinki, Finland; Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{J.~Budagov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{H.S.~Budd}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{K.~Burkett}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{G.~Busetto\ensuremath{^{ll}}}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, \ensuremath{^{ll}}University of Padova, I-35131 Padova, Italy}
\author{P.~Bussey}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{P.~Butti\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{A.~Buzatu}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{A.~Calamba}
\affiliation{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA}
\author{S.~Camarda}
\affiliation{Institut de Fisica d'Altes Energies, ICREA, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{M.~Campanelli}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{F.~Canelli\ensuremath{^{ee}}}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{B.~Carls}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{D.~Carlsmith}
\affiliation{University of Wisconsin-Madison, Madison, Wisconsin 53706, USA}
\author{R.~Carosi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{S.~Carrillo\ensuremath{^{l}}}
\affiliation{University of Florida, Gainesville, Florida 32611, USA}
\author{B.~Casal\ensuremath{^{j}}}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{M.~Casarsa}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{A.~Castro\ensuremath{^{kk}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{P.~Catastini}
\affiliation{Harvard University, Cambridge, Massachusetts 02138, USA}
\author{D.~Cauz\ensuremath{^{ss}}\ensuremath{^{tt}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{V.~Cavaliere}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{A.~Cerri\ensuremath{^{e}}}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{L.~Cerrito\ensuremath{^{r}}}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{Y.C.~Chen}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{M.~Chertok}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{G.~Chiarelli}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{G.~Chlachidze}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Cho}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{D.~Chokheli}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{A.~Clark}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{C.~Clarke}
\affiliation{Wayne State University, Detroit, Michigan 48201, USA}
\author{M.E.~Convery}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.~Conway}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{M.~Corbo\ensuremath{^{z}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Cordelli}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{C.A.~Cox}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{D.J.~Cox}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{M.~Cremonesi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{D.~Cruz}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{J.~Cuevas\ensuremath{^{y}}}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{R.~Culbertson}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{N.~d'Ascenzo\ensuremath{^{v}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Datta\ensuremath{^{hh}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~de~Barbaro}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{L.~Demortier}
\affiliation{The Rockefeller University, New York, New York 10065, USA}
\author{M.~Deninno}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{M.~D'Errico\ensuremath{^{ll}}}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, \ensuremath{^{ll}}University of Padova, I-35131 Padova, Italy}
\author{F.~Devoto}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki, FIN-00014, Helsinki, Finland; Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{A.~Di~Canto\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{B.~Di~Ruzza\ensuremath{^{p}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.R.~Dittmann}
\affiliation{Baylor University, Waco, Texas 76798, USA}
\author{S.~Donati\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{M.~D'Onofrio}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{M.~Dorigo\ensuremath{^{uu}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{A.~Driutti\ensuremath{^{ss}}\ensuremath{^{tt}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{K.~Ebina}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{R.~Edgar}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{R.~Erbacher}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{S.~Errede}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{B.~Esham}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{S.~Farrington}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{J.P.~Fern\'{a}ndez~Ramos}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{R.~Field}
\affiliation{University of Florida, Gainesville, Florida 32611, USA}
\author{G.~Flanagan\ensuremath{^{t}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{R.~Forrest}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{M.~Franklin}
\affiliation{Harvard University, Cambridge, Massachusetts 02138, USA}
\author{J.C.~Freeman}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Frisch}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{Y.~Funakoshi}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{C.~Galloni\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{A.F.~Garfinkel}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{P.~Garosi\ensuremath{^{nn}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{H.~Gerberich}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{E.~Gerchtein}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Giagu}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, \ensuremath{^{rr}}Sapienza Universit\`{a} di Roma, I-00185 Roma, Italy}
\author{V.~Giakoumopoulou}
\affiliation{University of Athens, 157 71 Athens, Greece}
\author{K.~Gibson}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, USA}
\author{C.M.~Ginsburg}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{N.~Giokaris}
\affiliation{University of Athens, 157 71 Athens, Greece}
\author{P.~Giromini}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{V.~Glagolev}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{D.~Glenzinski}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Gold}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131, USA}
\author{D.~Goldin}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{A.~Golossanov}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{G.~Gomez}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{G.~Gomez-Ceballos}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts 02139, USA}
\author{M.~Goncharov}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts 02139, USA}
\author{O.~Gonz\'{a}lez~L\'{o}pez}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{I.~Gorelov}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131, USA}
\author{A.T.~Goshaw}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{K.~Goulianos}
\affiliation{The Rockefeller University, New York, New York 10065, USA}
\author{E.~Gramellini}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{C.~Grosso-Pilcher}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{J.~Guimaraes~da~Costa}
\affiliation{Harvard University, Cambridge, Massachusetts 02138, USA}
\author{S.R.~Hahn}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.Y.~Han}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{F.~Happacher}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{K.~Hara}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{M.~Hare}
\affiliation{Tufts University, Medford, Massachusetts 02155, USA}
\author{R.F.~Harr}
\affiliation{Wayne State University, Detroit, Michigan 48201, USA}
\author{T.~Harrington-Taber\ensuremath{^{m}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Hatakeyama}
\affiliation{Baylor University, Waco, Texas 76798, USA}
\author{C.~Hays}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{J.~Heinrich}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{M.~Herndon}
\affiliation{University of Wisconsin-Madison, Madison, Wisconsin 53706, USA}
\author{A.~Hocker}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{Z.~Hong}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{W.~Hopkins\ensuremath{^{f}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Hou}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{R.E.~Hughes}
\affiliation{The Ohio State University, Columbus, Ohio 43210, USA}
\author{U.~Husemann}
\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{M.~Hussein\ensuremath{^{cc}}}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{J.~Huston}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{G.~Introzzi\ensuremath{^{pp}}\ensuremath{^{qq}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{M.~Iori\ensuremath{^{rr}}}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, \ensuremath{^{rr}}Sapienza Universit\`{a} di Roma, I-00185 Roma, Italy}
\author{A.~Ivanov\ensuremath{^{o}}}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{E.~James}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Jang}
\affiliation{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA}
\author{B.~Jayatilaka}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{E.J.~Jeon}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{S.~Jindariani}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Jones}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{K.K.~Joo}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{S.Y.~Jun}
\affiliation{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA}
\author{T.R.~Junk}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Kambeitz}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Karlsruhe Institute of Technology, D-76131 Karlsruhe, Germany}
\author{T.~Kamon}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{P.E.~Karchin}
\affiliation{Wayne State University, Detroit, Michigan 48201, USA}
\author{A.~Kasmi}
\affiliation{Baylor University, Waco, Texas 76798, USA}
\author{Y.~Kato\ensuremath{^{n}}}
\affiliation{Osaka City University, Osaka 558-8585, Japan}
\author{W.~Ketchum\ensuremath{^{ii}}}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{J.~Keung}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{B.~Kilminster\ensuremath{^{ee}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.H.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{H.S.~Kim\ensuremath{^{bb}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.E.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{M.J.~Kim}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{S.H.~Kim}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{S.B.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{Y.J.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{Y.K.~Kim}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{N.~Kimura}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{M.~Kirby}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Kondo}
\thanks{Deceased}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{D.J.~Kong}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{J.~Konigsberg}
\affiliation{University of Florida, Gainesville, Florida 32611, USA}
\author{A.V.~Kotwal}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{M.~Kreps}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Karlsruhe Institute of Technology, D-76131 Karlsruhe, Germany}
\author{J.~Kroll}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{M.~Kruse}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{T.~Kuhr}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Karlsruhe Institute of Technology, D-76131 Karlsruhe, Germany}
\author{M.~Kurata}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{A.T.~Laasanen}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{S.~Lammel}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Lancaster}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{K.~Lannon\ensuremath{^{x}}}
\affiliation{The Ohio State University, Columbus, Ohio 43210, USA}
\author{G.~Latino\ensuremath{^{nn}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{H.S.~Lee}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{J.S.~Lee}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{S.~Leo}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{S.~Leone}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{J.D.~Lewis}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Limosani\ensuremath{^{s}}}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{E.~Lipeles}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{A.~Lister\ensuremath{^{a}}}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{Q.~Liu}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{T.~Liu}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Lockwitz}
\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{A.~Loginov}
\affiliation{Yale University, New Haven, Connecticut 06520, USA}
\author{D.~Lucchesi\ensuremath{^{ll}}}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, \ensuremath{^{ll}}University of Padova, I-35131 Padova, Italy}
\author{A.~Luc\`{a}}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{J.~Lueck}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Karlsruhe Institute of Technology, D-76131 Karlsruhe, Germany}
\author{P.~Lujan}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{P.~Lukens}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{G.~Lungu}
\affiliation{The Rockefeller University, New York, New York 10065, USA}
\author{J.~Lys}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{R.~Lysak\ensuremath{^{d}}}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{R.~Madrak}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Maestro\ensuremath{^{nn}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{O.~Majersky}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{S.~Malik}
\affiliation{The Rockefeller University, New York, New York 10065, USA}
\author{G.~Manca\ensuremath{^{b}}}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{A.~Manousakis-Katsikakis}
\affiliation{University of Athens, 157 71 Athens, Greece}
\author{L.~Marchese\ensuremath{^{jj}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{F.~Margaroli}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, \ensuremath{^{rr}}Sapienza Universit\`{a} di Roma, I-00185 Roma, Italy}
\author{P.~Marino\ensuremath{^{oo}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{K.~Matera}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{M.E.~Mattson}
\affiliation{Wayne State University, Detroit, Michigan 48201, USA}
\author{A.~Mazzacane}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Mazzanti}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{R.~McNulty\ensuremath{^{i}}}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{A.~Mehta}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{P.~Mehtala}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki, FIN-00014, Helsinki, Finland; Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{C.~Mesropian}
\affiliation{The Rockefeller University, New York, New York 10065, USA}
\author{T.~Miao}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Mietlicki}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{A.~Mitra}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{H.~Miyake}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{S.~Moed}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{N.~Moggi}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{C.S.~Moon\ensuremath{^{z}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{R.~Moore\ensuremath{^{ff}}\ensuremath{^{gg}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.J.~Morello\ensuremath{^{oo}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{A.~Mukherjee}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{Th.~Muller}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Karlsruhe Institute of Technology, D-76131 Karlsruhe, Germany}
\author{P.~Murat}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Mussini\ensuremath{^{kk}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{J.~Nachtman\ensuremath{^{m}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{Y.~Nagai}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{J.~Naganoma}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{I.~Nakano}
\affiliation{Okayama University, Okayama 700-8530, Japan}
\author{A.~Napier}
\affiliation{Tufts University, Medford, Massachusetts 02155, USA}
\author{J.~Nett}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{T.~Nigmanov}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, USA}
\author{L.~Nodulman}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\author{S.Y.~Noh}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{O.~Norniella}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{L.~Oakes}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{S.H.~Oh}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{Y.D.~Oh}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{T.~Okusawa}
\affiliation{Osaka City University, Osaka 558-8585, Japan}
\author{R.~Orava}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki, FIN-00014, Helsinki, Finland; Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{L.~Ortolan}
\affiliation{Institut de Fisica d'Altes Energies, ICREA, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{C.~Pagliarone}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{E.~Palencia\ensuremath{^{e}}}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{P.~Palni}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131, USA}
\author{V.~Papadimitriou}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{W.~Parker}
\affiliation{University of Wisconsin-Madison, Madison, Wisconsin 53706, USA}
\author{G.~Pauletta\ensuremath{^{ss}}\ensuremath{^{tt}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{M.~Paulini}
\affiliation{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA}
\author{C.~Paus}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts 02139, USA}
\author{T.J.~Phillips}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{G.~Piacentino\ensuremath{^{q}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{E.~Pianori}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{J.~Pilot}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{K.~Pitts}
\affiliation{University of Illinois, Urbana, Illinois 61801, USA}
\author{C.~Plager}
\affiliation{University of California, Los Angeles, Los Angeles, California 90024, USA}
\author{L.~Pondrom}
\affiliation{University of Wisconsin-Madison, Madison, Wisconsin 53706, USA}
\author{S.~Poprocki\ensuremath{^{f}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Potamianos}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{A.~Pranko}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{F.~Prokoshin\ensuremath{^{aa}}}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{F.~Ptohos\ensuremath{^{g}}}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{G.~Punzi\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{I.~Redondo~Fern\'{a}ndez}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{P.~Renton}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{M.~Rescigno}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, \ensuremath{^{rr}}Sapienza Universit\`{a} di Roma, I-00185 Roma, Italy}
\author{F.~Rimondi}
\thanks{Deceased}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}
\author{L.~Ristori}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Robson}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{T.~Rodriguez}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{S.~Rolli\ensuremath{^{h}}}
\affiliation{Tufts University, Medford, Massachusetts 02155, USA}
\author{M.~Ronzani\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{R.~Roser}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.L.~Rosner}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{F.~Ruffini\ensuremath{^{nn}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{A.~Ruiz}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{J.~Russ}
\affiliation{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA}
\author{V.~Rusu}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{W.K.~Sakumoto}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{Y.~Sakurai}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{L.~Santi\ensuremath{^{ss}}\ensuremath{^{tt}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{K.~Sato}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{V.~Saveliev\ensuremath{^{v}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Savoy-Navarro\ensuremath{^{z}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Schlabach}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{E.E.~Schmidt}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{T.~Schwarz}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{L.~Scodellaro}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{F.~Scuri}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{S.~Seidel}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131, USA}
\author{Y.~Seiya}
\affiliation{Osaka City University, Osaka 558-8585, Japan}
\author{A.~Semenov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{F.~Sforza\ensuremath{^{mm}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{S.Z.~Shalhout}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{T.~Shears}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{P.F.~Shepard}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, USA}
\author{M.~Shimojima\ensuremath{^{u}}}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{M.~Shochet}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{I.~Shreyber-Tecker}
\affiliation{Institution for Theoretical and Experimental Physics, ITEP, Moscow 117259, Russia}
\author{A.~Simonenko}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{K.~Sliwa}
\affiliation{Tufts University, Medford, Massachusetts 02155, USA}
\author{J.R.~Smith}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{F.D.~Snider}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Song}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, USA}
\author{V.~Sorin}
\affiliation{Institut de Fisica d'Altes Energies, ICREA, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{R.~St.~Denis}
\thanks{Deceased}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{M.~Stancari}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Stentz\ensuremath{^{w}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.~Strologas}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131, USA}
\author{Y.~Sudo}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{A.~Sukhanov}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{I.~Suslov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{K.~Takemasa}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{Y.~Takeuchi}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{J.~Tang}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637, USA}
\author{M.~Tecchio}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{P.K.~Teng}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{J.~Thom\ensuremath{^{f}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{E.~Thomson}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{V.~Thukral}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{D.~Toback}
\affiliation{Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, Texas 77843, USA}
\author{S.~Tokar}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{K.~Tollefson}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{T.~Tomura}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{D.~Tonelli\ensuremath{^{e}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Torre}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{D.~Torretta}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Totaro}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, \ensuremath{^{ll}}University of Padova, I-35131 Padova, Italy}
\author{M.~Trovato\ensuremath{^{oo}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{F.~Ukegawa}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{S.~Uozumi}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{F.~V\'{a}zquez\ensuremath{^{l}}}
\affiliation{University of Florida, Gainesville, Florida 32611, USA}
\author{G.~Velev}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{C.~Vellidis}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{C.~Vernieri\ensuremath{^{oo}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, \ensuremath{^{mm}}University of Pisa, \ensuremath{^{nn}}University of Siena, \ensuremath{^{oo}}Scuola Normale Superiore, I-56127 Pisa, Italy, \ensuremath{^{pp}}INFN Pavia, I-27100 Pavia, Italy, \ensuremath{^{qq}}University of Pavia, I-27100 Pavia, Italy}
\author{M.~Vidal}
\affiliation{Purdue University, West Lafayette, Indiana 47907, USA}
\author{R.~Vilar}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{J.~Viz\'{a}n\ensuremath{^{dd}}}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{M.~Vogel}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131, USA}
\author{G.~Volpi}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{P.~Wagner}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{R.~Wallny\ensuremath{^{j}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.M.~Wang}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{D.~Waters}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{W.C.~Wester~III}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Whiteson\ensuremath{^{c}}}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{A.B.~Wicklund}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439, USA}
\author{S.~Wilbur}
\affiliation{University of California, Davis, Davis, California 95616, USA}
\author{H.H.~Williams}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104, USA}
\author{J.S.~Wilson}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{P.~Wilson}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{B.L.~Winer}
\affiliation{The Ohio State University, Columbus, Ohio 43210, USA}
\author{P.~Wittich\ensuremath{^{f}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Wolbers}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Wolfe}
\affiliation{The Ohio State University, Columbus, Ohio 43210, USA}
\author{T.~Wright}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{X.~Wu}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{Z.~Wu}
\affiliation{Baylor University, Waco, Texas 76798, USA}
\author{K.~Yamamoto}
\affiliation{Osaka City University, Osaka 558-8585, Japan}
\author{D.~Yamato}
\affiliation{Osaka City University, Osaka 558-8585, Japan}
\author{T.~Yang}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{U.K.~Yang}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{Y.C.~Yang}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{W.-M.~Yao}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\author{G.P.~Yeh}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Yi\ensuremath{^{m}}}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.~Yoh}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Yorita}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{T.~Yoshida\ensuremath{^{k}}}
\affiliation{Osaka City University, Osaka 558-8585, Japan}
\author{G.B.~Yu}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{I.~Yu}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon 305-806, Korea; Chonnam National University, Gwangju 500-757, Korea; Chonbuk National University, Jeonju 561-756, Korea; Ewha Womans University, Seoul, 120-750, Korea}
\author{A.M.~Zanetti}
\affiliation{Istituto Nazionale di Fisica Nucleare Trieste, \ensuremath{^{ss}}Gruppo Collegato di Udine, \ensuremath{^{tt}}University of Udine, I-33100 Udine, Italy, \ensuremath{^{uu}}University of Trieste, I-34127 Trieste, Italy}
\author{Y.~Zeng}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{C.~Zhou}
\affiliation{Duke University, Durham, North Carolina 27708, USA}
\author{S.~Zucchelli\ensuremath{^{kk}}}
\affiliation{Istituto Nazionale di Fisica Nucleare Bologna, \ensuremath{^{kk}}University of Bologna, I-40127 Bologna, Italy}

\collaboration{CDF Collaboration}
\altaffiliation[With visitors from]{
\ensuremath{^{a}}University of British Columbia, Vancouver, BC V6T 1Z1, Canada,
\ensuremath{^{b}}Istituto Nazionale di Fisica Nucleare, Sezione di Cagliari, 09042 Monserrato (Cagliari), Italy,
\ensuremath{^{c}}University of California Irvine, Irvine, CA 92697, USA,
\ensuremath{^{d}}Institute of Physics, Academy of Sciences of the Czech Republic, 182~21, Czech Republic,
\ensuremath{^{e}}CERN, CH-1211 Geneva, Switzerland,
\ensuremath{^{f}}Cornell University, Ithaca, NY 14853, USA,
\ensuremath{^{g}}University of Cyprus, Nicosia CY-1678, Cyprus,
\ensuremath{^{h}}Office of Science, U.S. Department of Energy, Washington, DC 20585, USA,
\ensuremath{^{i}}University College Dublin, Dublin 4, Ireland,
\ensuremath{^{j}}ETH, 8092 Z\"{u}rich, Switzerland,
\ensuremath{^{k}}University of Fukui, Fukui City, Fukui Prefecture, Japan 910-0017,
\ensuremath{^{l}}Universidad Iberoamericana, Lomas de Santa Fe, M\'{e}xico, C.P. 01219, Distrito Federal,
\ensuremath{^{m}}University of Iowa, Iowa City, IA 52242, USA,
\ensuremath{^{n}}Kinki University, Higashi-Osaka City, Japan 577-8502,
\ensuremath{^{o}}Kansas State University, Manhattan, KS 66506, USA,
\ensuremath{^{p}}Brookhaven National Laboratory, Upton, NY 11973, USA,
\ensuremath{^{q}}Istituto Nazionale di Fisica Nucleare, Sezione di Lecce, Via Arnesano, I-73100 Lecce, Italy,
\ensuremath{^{r}}Queen Mary, University of London, London, E1 4NS, United Kingdom,
\ensuremath{^{s}}University of Melbourne, Victoria 3010, Australia,
\ensuremath{^{t}}Muons, Inc., Batavia, IL 60510, USA,
\ensuremath{^{u}}Nagasaki Institute of Applied Science, Nagasaki 851-0193, Japan,
\ensuremath{^{v}}National Research Nuclear University, Moscow 115409, Russia,
\ensuremath{^{w}}Northwestern University, Evanston, IL 60208, USA,
\ensuremath{^{x}}University of Notre Dame, Notre Dame, IN 46556, USA,
\ensuremath{^{y}}Universidad de Oviedo, E-33007 Oviedo, Spain,
\ensuremath{^{z}}CNRS-IN2P3, Paris, F-75205 France,
\ensuremath{^{aa}}Universidad Tecnica Federico Santa Maria, 110v Valparaiso, Chile,
\ensuremath{^{bb}}Sejong University, Seoul 143-747, Korea,
\ensuremath{^{cc}}The University of Jordan, Amman 11942, Jordan,
\ensuremath{^{dd}}Universite catholique de Louvain, 1348 Louvain-La-Neuve, Belgium,
\ensuremath{^{ee}}University of Z\"{u}rich, 8006 Z\"{u}rich, Switzerland,
\ensuremath{^{ff}}Massachusetts General Hospital, Boston, MA 02114 USA,
\ensuremath{^{gg}}Harvard Medical School, Boston, MA 02114 USA,
\ensuremath{^{hh}}Hampton University, Hampton, VA 23668, USA,
\ensuremath{^{ii}}Los Alamos National Laboratory, Los Alamos, NM 87544, USA,
\ensuremath{^{jj}}Universit\`{a} degli Studi di Napoli Federico II, I-80138 Napoli, Italy
}
\noaffiliation
% Last update: $Date: 2016/01/04 20:42:12 $

